FS-COCO: Towards Understanding of Freehand Sketches of Common Objects in Context

We advance sketch research to scenes with the first dataset of freehand scene sketches, FS-COCO. With practical applications in mind, we collect sketches that convey scene content well but can be sketched within a few minutes by a person with any sketching skills. Our dataset comprises 10,000 freehand scene vector sketches with per point space-time information by 100 non-expert individuals, offering both object- and scene-level abstraction. Each sketch is augmented with its text description. Using our dataset, we study for the first time the problem of fine-grained image retrieval from freehand scene sketches and sketch captions. We draw insights on: (i) Scene salience encoded in sketches using the strokes temporal order; (ii) Performance comparison of image retrieval from a scene sketch and an image caption; (iii) Complementarity of information in sketches and image captions, as well as the potential benefit of combining the two modalities. In addition, we extend a popular vector sketch LSTM-based encoder to handle sketches with larger complexity than was supported by previous work. Namely, we propose a hierarchical sketch decoder, which we leverage at a sketch-specific "pre-text" task. Our dataset enables for the first time research on freehand scene sketch understanding and its practical applications.

==> data_collection_backup_pinaki.tex <==
\section{Dataset Collection}
\label{sec: dataset-collection}
Targeting practical applications, we aimed to collect representative freehand scene sketches with object- and scene-levels of abstraction. 
Therefore, we define the following requirements towards collected sketches: (1) created by non-professionals, (2) fast to create, (3) recognizable, (4) paired with images, and (5) supplemented with sketch-captions.
% To propel research into scene sketch-based applications, analysis of visual abstraction, and sketching strategies, we introduce the first dataset of freehand scene sketches with space-time information of each sketch point. 
% Our dataset will encourage research on scene sketch to image generation, sketch vectorization, sketch-based retrieval and sketch understanding in general. 
% To drive out insights on connections between a scene sketch, a photo and their captions, we supplement each sketch with its textual description.





\paragraph{Data preparation}
We randomly select $10k$ photos from MS-COCO \cite{lin2014cocoCaption}, a standard benchmark dataset for scene understanding \cite{CLIP, deeplabv2, chen2021visualgpt}. 
Each photo in this dataset is accompanied by image captions \cite{lin2014cocoCaption} and semantic segmentation \cite{caesar2018cocostuff}.
Our selected subset of photos includes $72$ \emph{``things"} instances (well-defined foreground objects) and $78$ \emph{``stuff"} instances (background instances with potentially no specific or distinctive spatial extent or shape: e.g., ``trees", ``fence"), according to the classification introduced in \cite{caesar2018cocostuff}. 
We present detailed statistics in \cref{sec:compare}.


\paragraph{Task}
We built a custom web application\footnote{We will release the code for the annotation tool and backend-server script upon acceptance.} to engage $100$ participants, each annotating a distinct subset of $100$ photos.
Our objective is to collect easy-to-recognize freehand scene sketches drawn from memory, alike single-object sketches collected previously \cite{tu-berlin, sketchy}.
To imitate real world scenario of sketching from memory, following the practice of single object dataset collection, we showed a reference scene photo to a subject for a limited duration of $60$ seconds, determined through a series of pilot studies.
To ensure recognizable but not overly detailed drawings, we also put time limits on the duration of the sketching. 
We determined the optimal time limits through a series of pilot studies with 10 participants, which showed that 3 minutes were sufficient for participants to comfortably sketch recognizable scene sketches.
We allow repeated sketching attempts, with the subject making an average of {$1.7$} attempts.
Each attempt repeats the entire process of observing an image and drawing on a blank canvas.
Upon satisfaction with their sketch, we ask the same subject to describe their sketch in text. 
The instructions to write a sketch caption are similar to that of Lin \etal \cite{lin2014cocoCaption} and are provided in supplemental materials.
To reduce fatigue that can compromise data quality, we encourage participants to take frequent breaks and complete the task over multiple days. 
Thus, each participant spent $12-13$ hours to annotate $100$ photos over an average period of $2$ days.

\paragraph{Quality check}
We check the quality of sketches. 
We hired as a \emph{human judge} one appointed person (1) with experience in data collection and (2) non-expert in sketching.
The human judge instructed to "mark sketches of scenes that are \emph{too difficult to understand or recognize}."
The tagged photos were sent back to their assigned annotator. 
This process guarantees the resulting scene sketches are recognizable by a human, and therefore, should be understood by a machine.



\paragraph{Participants}
We recruited $100$ non-artist participants from the age group $22-44$, with tan average age of $27.03$, including $72$ males and $28$ females.
% \footnote{See supplemental for details on how consent was obtained.}. 

\section{Dataset composition}
\label{sec:data_categories}
Our dataset consists of $10,000$ (a) unique freehand scene sketches, (b) textual descriptions of the sketches (sketch captions), (c) reference photos from the MS-COCO \cite{lin2014cocoCaption} dataset.
Each photo in \cite{lin2014cocoCaption} contains 5 associated text descriptions (image captions) by different subjects \cite{lin2014cocoCaption}. 
\cref{fig:dataset-comparison,fig:sample-data} show samples from our dataset, and supplemental materials visualize more sketches from our dataset.

% \cref{fig:dataset-comparison,fig:sample-data} provide some samples from our dataset, while \cref{tab:datasets_comparison} provides comparison with previous dataset and statistics on distribution of object categories in our sketches. 
% The supplemental provides additional sketch examples and detailed statistics on object categories.
% \begin{table*}[t]
%     \centering
%     \caption{Comparison of scene sketch datasets based on the distribution of categories in sketch-image pairs. `FG' denotes subsets of datasets that are recommended for use in Fine-Grained tasks such as fine-grained retrieval that we study. `u/l' denotes upper and lower bounds for the number of categories for our dataset, see \cref{sec:data_categories} for details.}
% %    \vspace{-0.25cm}
% \scriptsize{
% % \resizebox{\linewidth}{!}{%
% \begin{tabular}{l|r|r|rrrr|rrrr}
% \multirow{2}{*}{Dataset} & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}$\#$ pho-\\ tos\end{tabular}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}$\#$cate-\\ gories\end{tabular}}} &  \multicolumn{4}{c|}{$\#$ categories per sketch}                                                           & \multicolumn{4}{c}{$\#$ sketches per category}                                                              \\
%                  &  & \multicolumn{1}{c|}{}                                                             & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c|}{Std}  & \multicolumn{1}{c}{Min} & \multicolumn{1}{c|}{Max} & 
%                          \multicolumn{1}{c}{Mean} & \multicolumn{1}{c|}{Std}     
%                          & \multicolumn{1}{c}{Min} & \multicolumn{1}{c}{Max} 
%                          \\ \hline
% \texttt{SketchyScene \cite{sketchyscene}}    & 7,264                                                                                                 & 45                                                                                               & 7.88                     & \multicolumn{1}{r|}{1.96} & 4                       & 20                       & 1087.02                  & \multicolumn{1}{r|}{1416.49} & 31                      & 5723                    \\
% \texttt{SketchyCOCO \cite{gao2020sketchyCOCO}}     & 14,081                                                                                        & 17                                                                                               & 3.33                     & \multicolumn{1}{r|}{0.9}  & 2                       & 7                        & 1932.41                  & \multicolumn{1}{r|}{3493.01} & 33                      & 9761                    \\ \hline
% \texttt{SketchyScene FG}    & 2,724 & 45                                                                                               & 7.71                     & \multicolumn{1}{r|}{1.88} & 4                       & 20                       & 397.65                  & \multicolumn{1}{r|}{528.85} & 3                      & 2154                   \\
% \texttt{SketchyCOCO FG}    &   1,225                                                                                                    & 17                                                                                               & 3.28                     & \multicolumn{1}{r|}{0.89}  & 2                       & 6                        & 164.71                  & \multicolumn{1}{r|}{297.79} & 5                      & 824                   \\
% \hline
% \textbf{FS-COCO} (l) & 10,000                                                                                        & 95                                                                                               & 1.37                     & \multicolumn{1}{r|}{0.57} & 1                       & 5                        & 89.72                    & \multicolumn{1}{r|}{159.9}   & 1                       & 853                     \\ 
% \textbf{FS-COCO} (u) & 10,000                                                                                        & 150                                                                                               & 7.17                     & \multicolumn{1}{r|}{3.27} & 1                       & 25                        & 413.18                    & \multicolumn{1}{r|}{973.59}   & 1                       & 6789                     \\ \hline
% \end{tabular}%
% % }
% }
%     \label{tab:datasets_comparison}
%      \vspace{-0.3cm}
% \end{table*}

\begin{table*}[t]
    \centering
    \caption{Comparison of scene sketch datasets based on the distribution of categories in sketch-image pairs. `FG' denotes subsets of datasets that are recommended for use in Fine-Grained tasks such as fine-grained retrieval that we study. `u/l' denotes upper and lower bounds for the number of categories for our dataset, see \cref{sec:data_categories} for details.}
%    \vspace{-0.25cm}
\scriptsize{
% \resizebox{\linewidth}{!}{%
\begin{tabular}{l|r|r|rrrr|rrrr}
\multirow{2}{*}{Dataset} & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}$\#$ pho-\\ tos\end{tabular}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}$\#$cate-\\ gories\end{tabular}}} &  \multicolumn{4}{c|}{$\#$ categories per sketch}                                                           & \multicolumn{4}{c}{$\#$ sketches per category}                                                              \\
                 &  & \multicolumn{1}{c|}{}                                                             & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c|}{Std}  & \multicolumn{1}{c}{Min} & \multicolumn{1}{c|}{Max} & 
                         \multicolumn{1}{c}{Mean} & \multicolumn{1}{c|}{Std}     
                         & \multicolumn{1}{c}{Min} & \multicolumn{1}{c}{Max} 
                         \\ \hline
\texttt{SketchyScene \cite{sketchyscene}}    & 7,264                                                                                                 & 45                                                                                               & 7.88                     & \multicolumn{1}{r|}{1.96} & 4                       & 20                       & 1079.76                  & \multicolumn{1}{r|}{1447.47} & 31                      & 5723                    \\
\texttt{SketchyCOCO \cite{gao2020sketchyCOCO}}     & 14,081                                                                                        & 17                                                                                               & 3.33                     & \multicolumn{1}{r|}{0.9}  & 2                       & 7                        & 1932.41                  & \multicolumn{1}{r|}{3493.01} & 33                      & 9761                    \\ \hline
\texttt{SketchyScene FG}    & 2,724 & 45                                                                                               & 7.71                     & \multicolumn{1}{r|}{1.88} & 4                       & 20                       & 394.51                  & \multicolumn{1}{r|}{540.30} & 3                      & 2154                   \\
\texttt{SketchyCOCO FG}    &   1,225                                                                                                    & 17                                                                                               & 3.28                     & \multicolumn{1}{r|}{0.89}  & 2                       & 6                        & 164.71                  & \multicolumn{1}{r|}{297.79} & 5                      & 824                   \\
\hline
\textbf{FS-COCO} (l) & 10,000                                                                                        & 95                                                                                               & 1.37                     & \multicolumn{1}{r|}{0.57} & 1                       & 5                        & 89.72                    & \multicolumn{1}{r|}{159.9}   & 1                       & 853                     \\ 
\textbf{FS-COCO} (u) & 10,000                                                                                        & 150                                                                                               & 7.17                     & \multicolumn{1}{r|}{3.27} & 1                       & 25                        & 413.18                    & \multicolumn{1}{r|}{973.59}   & 1                       & 6789                     \\ \hline
\end{tabular}%
% }
}
    \label{tab:datasets_comparison}
     \vspace{-0.3cm}
\end{table*}























% \begin{table*}[t]
%     \centering
%     \caption{Comparison of scene sketch datasets: \texttt{SketchyScene} \cite{sketchyscene}, \texttt{SketchyCOCO} \cite{gao2020sketchyCOCO} and \newDataset~(ours). \todo{Update the numbers, based on lower/upper bound?.}}
% %    \vspace{-0.25cm}
% %    \small{
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{c|cc|r|c|c|c|r|rrrr|rrrr}
% \multirow{2}{*}{Dataset} & \multicolumn{2}{c|}{Abstraction} & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}$\#$ pho-\\ tos\end{tabular}}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Vector \\ Sketch\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Cap-\\ tions\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Free-\\ hand\end{tabular}} & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}$\#$cate-\\ gories\end{tabular}}} & \multicolumn{4}{c|}{$\#$ categories per sketch}                                                           & \multicolumn{4}{c}{$\#$ sketches per category}                                                              \\
%                          & Object          & Scene          & \multicolumn{1}{c|}{}                                                                         &                                                                           &                                                                       &                                                                       & \multicolumn{1}{c|}{}                                                                            & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c|}{Std}  & \multicolumn{1}{c}{Min} & \multicolumn{1}{c|}{Max} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c|}{Std}     & \multicolumn{1}{c}{Min} & \multicolumn{1}{c}{Max} \\ \hline
% \texttt{SketchyScene}    & \textcolor{PineGreen}{\cmark}         & \xmark         & 7,264                                                                                         & \xmark                                                                    & \xmark                                                                & \xmark                                                                & 45                                                                                               & 7.88                     & \multicolumn{1}{r|}{1.96} & 4                       & 20                       & 1087.02                  & \multicolumn{1}{r|}{1416.49} & 31                      & 5723                    \\
% \texttt{SketchyCOCO}     & \xmark          & \textcolor{PineGreen}{\cmark}        & 14,081                                                                                        & \xmark                                                                    & \xmark                                                                & \xmark                                                                & 17                                                                                               & 3.33                     & \multicolumn{1}{r|}{0.9}  & 2                       & 7                        & 1932.41                  & \multicolumn{1}{r|}{3388.72} & 33                      & 9761                    \\
% \textbf{FS-COCO}  & \textcolor{PineGreen}{\cmark}         & \textcolor{PineGreen}{\cmark}        & 10,000                                                                                        & \textcolor{PineGreen}{\cmark}                                                                   & \textcolor{PineGreen}{\cmark}                                                               & \textcolor{PineGreen}{\cmark}                                                               & 95                                                                                               & 1.37/7.17                     & \multicolumn{1}{r|}{0.57/3.27} & 1/1                       & 5/25                        & 89.72/413.18                    & \multicolumn{1}{r|}{159.9/973.59}   & 1/1                       & 853/6789                     \\ \hline
% \end{tabular}%
% }
% %    }
%     \label{tab:datasets_comparison}
%      \vspace{-0.3cm}
% \end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{table*}[t]
%     \centering
%     \caption{Comparison of scene sketch datasets: \texttt{SketchyScene} \cite{sketchyscene}, \texttt{SketchyCOCO} \cite{gao2020sketchyCOCO} and \newDataset~(ours). \todo{Update the numbers, based on lower/upper bound?.} Using training/testing set for retrieval}
% %    \vspace{-0.25cm}
% %    \small{
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{c|cc|r|c|c|c|r|rrrr|rrrr}
% \multirow{2}{*}{Dataset} & \multicolumn{2}{c|}{Abstraction} & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}$\#$ pho-\\ tos\end{tabular}}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Vector \\ Sketch\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Cap-\\ tions\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Free-\\ hand\end{tabular}} & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}$\#$cate-\\ gories\end{tabular}}} & \multicolumn{4}{c|}{$\#$ categories per sketch}                                                           & \multicolumn{4}{c}{$\#$ sketches per category}                                                              \\
%                          & Object          & Scene          & \multicolumn{1}{c|}{}                                                                         &                                                                           &                                                                       &                                                                       & \multicolumn{1}{c|}{}                                                                            & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c|}{Std}  & \multicolumn{1}{c}{Min} & \multicolumn{1}{c|}{Max} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c|}{Std}     & \multicolumn{1}{c}{Min} & \multicolumn{1}{c}{Max} \\ \hline
% \texttt{SketchyScene}    & \textcolor{PineGreen}{\cmark}         & \xmark         & 2,724                                                                                         & \xmark                                                                    & \xmark                                                                & \xmark                                                                & 45                                                                                               & 7.71                     & \multicolumn{1}{r|}{1.88} & 4                       & 20                       & 397.65                  & \multicolumn{1}{r|}{528.85} & 3                      & 2154                    \\
% \texttt{SketchyCOCO}     & \xmark          & \textcolor{PineGreen}{\cmark}        & 1,225                                                                                        & \xmark                                                                    & \xmark                                                                & \xmark                                                                & 17                                                                                               & 3.28                     & \multicolumn{1}{r|}{0.89}  & 2                       & 6                        & 164.71                  & \multicolumn{1}{r|}{288.89} & 5                      & 824                    \\ \hline
% \end{tabular}%
% }
% %    }
%     \label{tab:datasets_comparison_retrieval}
%      \vspace{-0.3cm}
% \end{table*}

\subsection{Comparison to existing datasets}
\label{sec:compare}

\cref{tab:datasets_comparison} provides comparison with previous dataset and statistics on distribution of object categories in our sketches, which we discuss in more detail below. 

\paragraph{Categories} 
First, we obtain a joint set of labels from the labels in \cite{sketchyscene,gao2020sketchyCOCO} and \cite{caesar2018cocostuff}. 
To compute statistics on the categories present in \cite{sketchyscene,gao2020sketchyCOCO}, we use the semantic segmentation labels available in these datasets. 
For our dataset, we compute two estimates of the category distribution across our data: (1) based on semantic segmentation labels in images and (2) based on the occurrence of a word in a sketch caption. 
As can be seen from \cref{fig:sample-data}, the participants do not exhaustively describe in the caption all the objects present in sketches. 
The first constitutes the upper estimate $u$, and the second the lower estimate $l$.
Our dataset contains $l/u=95/150$ categories, which is more than double the number of categories in previous scene sketch datasets (\cref{tab:datasets_comparison}). 
On average, each category is present in $l/u=89.72/413.18$ sketches.
% \cref{fig:categories} shows the distribution of categories over the three datasets.
Among the most common category in all three datasets are `cloud', `tree' and `grass'  common to outdoor scenes. 
% The most common categories for our dataset are `grass', `tree' and `road' common to outdoor scenes. 
In our dataset `person' is also among one of the most frequent categories along with common animals such as `horse', `giraffe', `dog', `cow' and `sheep'. 
Our dataset, according to lower/upper estimates, contains $27$/$71$ indoor categories and $53$/$79$ outdoor categories.
We provide detailed statistics in supplemental materials. 

\paragraph{Sketch complexity} 
Existing datasets of freehand sketches \cite{tu-berlin, sketchy} contain sketches of single objects. 
The complexity of scene sketches is unavoidably higher than the one of single-object sketches.
Sketches in our dataset have a median stroke count of $64$.
For comparison, a median strokes count in the popular \texttt{Tu-Berlin} \cite{tu-berlin} and \texttt{Sketchy} \cite{sketchy} datasets is $13$ and $14$, respectively.

==> dataset_collection.tex <==
\section{Dataset Collection}
\label{sec: dataset-collection}
Targeting practical applications, we aimed to collect representative freehand scene sketches with object- and scene-levels of abstraction. 
Therefore, we define the following requirements towards collected sketches: (1) created by non-professionals, (2) fast to create, (3) recognizable, (4) paired with images, and (5) supplemented with sketch-captions.
% To propel research into scene sketch-based applications, analysis of visual abstraction, and sketching strategies, we introduce the first dataset of freehand scene sketches with space-time information of each sketch point. 
% Our dataset will encourage research on scene sketch to image generation, sketch vectorization, sketch-based retrieval and sketch understanding in general. 
% To drive out insights on connections between a scene sketch, a photo and their captions, we supplement each sketch with its textual description.





\paragraph{Data preparation}
We randomly select $10k$ photos from MS-COCO \cite{lin2014cocoCaption}, a standard benchmark dataset for scene understanding \cite{CLIP, deeplabv2, chen2021visualgpt}. 
Each photo in this dataset is accompanied by image captions \cite{lin2014cocoCaption} and semantic segmentation \cite{caesar2018cocostuff}.
Our selected subset of photos includes $72$ \emph{``things"} instances (well-defined foreground objects) and $78$ \emph{``stuff"} instances (background instances with potentially no specific or distinctive spatial extent or shape: e.g., ``trees", ``fence"), according to the classification introduced in \cite{caesar2018cocostuff}. 
We present detailed statistics in \cref{sec:compare}.


\paragraph{Task}
We built a custom web application\footnote{We will release the code for the annotation tool and backend-server script upon acceptance.} to engage $100$ participants, each annotating a distinct subset of $100$ photos.
Our objective is to collect easy-to-recognize freehand scene sketches drawn from memory, alike single-object sketches collected previously \cite{tu-berlin, sketchy}.
To imitate real world scenario of sketching from memory, following the practice of single object dataset collection, we showed a reference scene photo to a subject for a limited duration of $60$ seconds, determined through a series of pilot studies.
To ensure recognizable but not overly detailed drawings, we also put time limits on the duration of the sketching. 
We determined the optimal time limits through a series of pilot studies with 10 participants, which showed that 3 minutes were sufficient for participants to comfortably sketch recognizable scene sketches.
We allow repeated sketching attempts, with the subject making an average of {$1.7$} attempts.
Each attempt repeats the entire process of observing an image and drawing on a blank canvas.
Upon satisfaction with their sketch, we ask the same subject to describe their sketch in text. 
The instructions to write a sketch caption are similar to that of Lin \etal \cite{lin2014cocoCaption} and are provided in supplemental materials.
To reduce fatigue that can compromise data quality, we encourage participants to take frequent breaks and complete the task over multiple days. 
Thus, each participant spent $12-13$ hours to annotate $100$ photos over an average period of $2$ days.

\paragraph{Quality check}
We check the quality of sketches. 
We hired as a \emph{human judge} one appointed person (1) with experience in data collection and (2) non-expert in sketching.
The human judge instructed to ``mark sketches of scenes that are \emph{too difficult to understand or recognize}."
The tagged photos were sent back to their assigned annotator. 
This process guarantees the resulting scene sketches are recognizable by a human, and therefore, should be understood by a machine.



\paragraph{Participants}
We recruited $100$ non-artist participants from the age group $22-44$, with an average age of $27.03$, including $72$ males and $28$ females.
% \footnote{See supplemental for details on how consent was obtained.}. 

\section{Dataset composition}
\label{sec:data_categories}
Our dataset consists of $10,000$ (a) unique freehand scene sketches, (b) textual descriptions of the sketches (sketch captions), (c) reference photos from the MS-COCO \cite{lin2014cocoCaption} dataset.
Each photo in \cite{lin2014cocoCaption} contains 5 associated text descriptions (image captions) by different subjects \cite{lin2014cocoCaption}. 
\cref{fig:dataset-comparison,fig:sample-data} show samples from our dataset, and supplemental materials visualize more sketches from our dataset.

% \cref{fig:dataset-comparison,fig:sample-data} provide some samples from our dataset, while \cref{tab:datasets_comparison} provides comparison with previous dataset and statistics on distribution of object categories in our sketches. 
% The supplemental provides additional sketch examples and detailed statistics on object categories.
% \begin{table*}[t]
%     \centering
%     \caption{Comparison of scene sketch datasets based on the distribution of categories in sketch-image pairs. `FG' denotes subsets of datasets that are recommended for use in Fine-Grained tasks such as fine-grained retrieval that we study. `u/l' denotes upper and lower bounds for the number of categories for our dataset, see \cref{sec:data_categories} for details.}
% %    \vspace{-0.25cm}
% \scriptsize{
% % \resizebox{\linewidth}{!}{%
% \begin{tabular}{l|r|r|rrrr|rrrr}
% \multirow{2}{*}{Dataset} & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}$\#$ pho-\\ tos\end{tabular}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}$\#$cate-\\ gories\end{tabular}}} &  \multicolumn{4}{c|}{$\#$ categories per sketch}                                                           & \multicolumn{4}{c}{$\#$ sketches per category}                                                              \\
%                  &  & \multicolumn{1}{c|}{}                                                             & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c|}{Std}  & \multicolumn{1}{c}{Min} & \multicolumn{1}{c|}{Max} & 
%                          \multicolumn{1}{c}{Mean} & \multicolumn{1}{c|}{Std}     
%                          & \multicolumn{1}{c}{Min} & \multicolumn{1}{c}{Max} 
%                          \\ \hline
% \texttt{SketchyScene \cite{sketchyscene}}    & 7,264                                                                                                 & 45                                                                                               & 7.88                     & \multicolumn{1}{r|}{1.96} & 4                       & 20                       & 1087.02                  & \multicolumn{1}{r|}{1416.49} & 31                      & 5723                    \\
% \texttt{SketchyCOCO \cite{gao2020sketchyCOCO}}     & 14,081                                                                                        & 17                                                                                               & 3.33                     & \multicolumn{1}{r|}{0.9}  & 2                       & 7                        & 1932.41                  & \multicolumn{1}{r|}{3493.01} & 33                      & 9761                    \\ \hline
% \texttt{SketchyScene FG}    & 2,724 & 45                                                                                               & 7.71                     & \multicolumn{1}{r|}{1.88} & 4                       & 20                       & 397.65                  & \multicolumn{1}{r|}{528.85} & 3                      & 2154                   \\
% \texttt{SketchyCOCO FG}    &   1,225                                                                                                    & 17                                                                                               & 3.28                     & \multicolumn{1}{r|}{0.89}  & 2                       & 6                        & 164.71                  & \multicolumn{1}{r|}{297.79} & 5                      & 824                   \\
% \hline
% \textbf{FS-COCO} (l) & 10,000                                                                                        & 95                                                                                               & 1.37                     & \multicolumn{1}{r|}{0.57} & 1                       & 5                        & 89.72                    & \multicolumn{1}{r|}{159.9}   & 1                       & 853                     \\ 
% \textbf{FS-COCO} (u) & 10,000                                                                                        & 150                                                                                               & 7.17                     & \multicolumn{1}{r|}{3.27} & 1                       & 25                        & 413.18                    & \multicolumn{1}{r|}{973.59}   & 1                       & 6789                     \\ \hline
% \end{tabular}%
% % }
% }
%     \label{tab:datasets_comparison}
%      \vspace{-0.3cm}
% \end{table*}

\begin{table*}[t]
    \centering
    \caption{Comparison of scene sketch datasets based on the distribution of categories in sketch-image pairs. `FG' denotes subsets of datasets that are recommended for use in Fine-Grained tasks such as fine-grained retrieval that we study. `u/l' denotes upper and lower bounds for the number of categories for our dataset, see \cref{sec:data_categories} for details.}
%    \vspace{-0.25cm}
\scriptsize{
% \resizebox{\linewidth}{!}{%
\begin{tabular}{l|r|r|rrrr|rrrr}
\multirow{2}{*}{Dataset} & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}$\#$ pho-\\ tos\end{tabular}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}$\#$cate-\\ gories\end{tabular}}} &  \multicolumn{4}{c|}{$\#$ categories per sketch}                                                           & \multicolumn{4}{c}{$\#$ sketches per category}                                                              \\
                 &  & \multicolumn{1}{c|}{}                                                             & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c|}{Std}  & \multicolumn{1}{c}{Min} & \multicolumn{1}{c|}{Max} & 
                         \multicolumn{1}{c}{Mean} & \multicolumn{1}{c|}{Std}     
                         & \multicolumn{1}{c}{Min} & \multicolumn{1}{c}{Max} 
                         \\ \hline
\texttt{SketchyScene \cite{sketchyscene}}    & 7,264                                                                                                 & 45                                                                                               & 7.88                     & \multicolumn{1}{r|}{1.96} & 4                       & 20                       & 1079.76                  & \multicolumn{1}{r|}{1447.47} & 31                      & 5723                    \\
\texttt{SketchyCOCO \cite{gao2020sketchyCOCO}}     & 14,081                                                                                        & 17                                                                                               & 3.33                     & \multicolumn{1}{r|}{0.9}  & 2                       & 7                        & 1932.41                  & \multicolumn{1}{r|}{3493.01} & 33                      & 9761                    \\ \hline
\texttt{SketchyScene FG}    & 2,724 & 45                                                                                               & 7.71                     & \multicolumn{1}{r|}{1.88} & 4                       & 20                       & 394.51                  & \multicolumn{1}{r|}{540.30} & 3                      & 2154                   \\
\texttt{SketchyCOCO FG}    &   1,225                                                                                                    & 17                                                                                               & 3.28                     & \multicolumn{1}{r|}{0.89}  & 2                       & 6                        & 164.71                  & \multicolumn{1}{r|}{297.79} & 5                      & 824                   \\
\hline
\textbf{FS-COCO} (l) & 10,000                                                                                        & 92                                                                                               & 1.37                     & \multicolumn{1}{r|}{0.57} & 1                       & 5                        & 99.42                    & \multicolumn{1}{r|}{172.88}   & 1                       & 866                     \\ 
\textbf{FS-COCO} (u) & 10,000                                                                                        & 150                                                                                               & 7.17                     & \multicolumn{1}{r|}{3.27} & 1                       & 25                        & 413.18                    & \multicolumn{1}{r|}{973.59}   & 1                       & 6789                     \\ \hline
\end{tabular}%
% }
}
    \label{tab:datasets_comparison}
     \vspace{-0.3cm}
\end{table*}























% \begin{table*}[t]
%     \centering
%     \caption{Comparison of scene sketch datasets: \texttt{SketchyScene} \cite{sketchyscene}, \texttt{SketchyCOCO} \cite{gao2020sketchyCOCO} and \newDataset~(ours). \todo{Update the numbers, based on lower/upper bound?.}}
% %    \vspace{-0.25cm}
% %    \small{
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{c|cc|r|c|c|c|r|rrrr|rrrr}
% \multirow{2}{*}{Dataset} & \multicolumn{2}{c|}{Abstraction} & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}$\#$ pho-\\ tos\end{tabular}}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Vector \\ Sketch\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Cap-\\ tions\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Free-\\ hand\end{tabular}} & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}$\#$cate-\\ gories\end{tabular}}} & \multicolumn{4}{c|}{$\#$ categories per sketch}                                                           & \multicolumn{4}{c}{$\#$ sketches per category}                                                              \\
%                          & Object          & Scene          & \multicolumn{1}{c|}{}                                                                         &                                                                           &                                                                       &                                                                       & \multicolumn{1}{c|}{}                                                                            & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c|}{Std}  & \multicolumn{1}{c}{Min} & \multicolumn{1}{c|}{Max} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c|}{Std}     & \multicolumn{1}{c}{Min} & \multicolumn{1}{c}{Max} \\ \hline
% \texttt{SketchyScene}    & \textcolor{PineGreen}{\cmark}         & \xmark         & 7,264                                                                                         & \xmark                                                                    & \xmark                                                                & \xmark                                                                & 45                                                                                               & 7.88                     & \multicolumn{1}{r|}{1.96} & 4                       & 20                       & 1087.02                  & \multicolumn{1}{r|}{1416.49} & 31                      & 5723                    \\
% \texttt{SketchyCOCO}     & \xmark          & \textcolor{PineGreen}{\cmark}        & 14,081                                                                                        & \xmark                                                                    & \xmark                                                                & \xmark                                                                & 17                                                                                               & 3.33                     & \multicolumn{1}{r|}{0.9}  & 2                       & 7                        & 1932.41                  & \multicolumn{1}{r|}{3388.72} & 33                      & 9761                    \\
% \textbf{FS-COCO}  & \textcolor{PineGreen}{\cmark}         & \textcolor{PineGreen}{\cmark}        & 10,000                                                                                        & \textcolor{PineGreen}{\cmark}                                                                   & \textcolor{PineGreen}{\cmark}                                                               & \textcolor{PineGreen}{\cmark}                                                               & 95                                                                                               & 1.37/7.17                     & \multicolumn{1}{r|}{0.57/3.27} & 1/1                       & 5/25                        & 89.72/413.18                    & \multicolumn{1}{r|}{159.9/973.59}   & 1/1                       & 853/6789                     \\ \hline
% \end{tabular}%
% }
% %    }
%     \label{tab:datasets_comparison}
%      \vspace{-0.3cm}
% \end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{table*}[t]
%     \centering
%     \caption{Comparison of scene sketch datasets: \texttt{SketchyScene} \cite{sketchyscene}, \texttt{SketchyCOCO} \cite{gao2020sketchyCOCO} and \newDataset~(ours). \todo{Update the numbers, based on lower/upper bound?.} Using training/testing set for retrieval}
% %    \vspace{-0.25cm}
% %    \small{
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{c|cc|r|c|c|c|r|rrrr|rrrr}
% \multirow{2}{*}{Dataset} & \multicolumn{2}{c|}{Abstraction} & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}$\#$ pho-\\ tos\end{tabular}}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Vector \\ Sketch\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Cap-\\ tions\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Free-\\ hand\end{tabular}} & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}$\#$cate-\\ gories\end{tabular}}} & \multicolumn{4}{c|}{$\#$ categories per sketch}                                                           & \multicolumn{4}{c}{$\#$ sketches per category}                                                              \\
%                          & Object          & Scene          & \multicolumn{1}{c|}{}                                                                         &                                                                           &                                                                       &                                                                       & \multicolumn{1}{c|}{}                                                                            & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c|}{Std}  & \multicolumn{1}{c}{Min} & \multicolumn{1}{c|}{Max} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c|}{Std}     & \multicolumn{1}{c}{Min} & \multicolumn{1}{c}{Max} \\ \hline
% \texttt{SketchyScene}    & \textcolor{PineGreen}{\cmark}         & \xmark         & 2,724                                                                                         & \xmark                                                                    & \xmark                                                                & \xmark                                                                & 45                                                                                               & 7.71                     & \multicolumn{1}{r|}{1.88} & 4                       & 20                       & 397.65                  & \multicolumn{1}{r|}{528.85} & 3                      & 2154                    \\
% \texttt{SketchyCOCO}     & \xmark          & \textcolor{PineGreen}{\cmark}        & 1,225                                                                                        & \xmark                                                                    & \xmark                                                                & \xmark                                                                & 17                                                                                               & 3.28                     & \multicolumn{1}{r|}{0.89}  & 2                       & 6                        & 164.71                  & \multicolumn{1}{r|}{288.89} & 5                      & 824                    \\ \hline
% \end{tabular}%
% }
% %    }
%     \label{tab:datasets_comparison_retrieval}
%      \vspace{-0.3cm}
% \end{table*}

\subsection{Comparison to existing datasets}
\label{sec:compare}

\cref{tab:datasets_comparison} provides comparison with previous dataset and statistics on distribution of object categories in our sketches, which we discuss in more detail below. 

\paragraph{Categories} 
First, we obtain a joint set of labels from the labels in \cite{sketchyscene,gao2020sketchyCOCO} and \cite{caesar2018cocostuff}. 
To compute statistics on the categories present in \cite{sketchyscene,gao2020sketchyCOCO}, we use the semantic segmentation labels available in these datasets. 
For our dataset, we compute two estimates of the category distribution across our data: (1) based on semantic segmentation labels in images and (2) based on the occurrence of a word in a sketch caption. 
As can be seen from \cref{fig:sample-data}, the participants do not exhaustively describe in the caption all the objects present in sketches. 
The first constitutes the upper estimate $u$, and the second the lower estimate $l$.
Our dataset contains $l/u=92/150$ categories, which is more than double the number of categories in previous scene sketch datasets (\cref{tab:datasets_comparison}). 
On average, each category is present in $l/u=99.42/413.18$ sketches.
% \cref{fig:categories} shows the distribution of categories over the three datasets.
Among the most common category in all three datasets are `cloud', `tree' and `grass'  common to outdoor scenes. 
% The most common categories for our dataset are `grass', `tree' and `road' common to outdoor scenes. 
In our dataset `person' is also among one of the most frequent categories along with common animals such as `horse', `giraffe', `dog', `cow' and `sheep'. 
Our dataset, according to lower/upper estimates, contains $33$/$71$ indoor categories and $59$/$79$ outdoor categories.
We provide detailed statistics in supplemental materials. 

\paragraph{Sketch complexity} 
Existing datasets of freehand sketches \cite{tu-berlin, sketchy} contain sketches of single objects. 
The complexity of scene sketches is unavoidably higher than the one of single-object sketches.
Sketches in our dataset have a median stroke count of $64$.
For comparison, a median strokes count in the popular \texttt{Tu-Berlin} \cite{tu-berlin} and \texttt{Sketchy} \cite{sketchy} datasets is $13$ and $14$, respectively.

==> eccv_copy/dataset_collection.tex <==
\section{Dataset Collection}
\label{sec: dataset-collection}
Targeting practical applications, we aimed to collect freehand scene sketches with object- and scene-levels of abstraction. Therefore, we define the following requirements towards collected sketches: (1) created by non-professionals, (2) fast to create, (3) recognizable, (4) paired with images, and (5) supplemented with sketch-captions.
% To propel research into scene sketch-based applications, analysis of visual abstraction, and sketching strategies, we introduce the first dataset of freehand scene sketches with space-time information of each sketch point. 
% Our dataset will encourage research on scene sketch to image generation, sketch vectorization, sketch-based retrieval and sketch understanding in general. 
% To drive out insights on connections between a scene sketch, a photo and their captions, we supplement each sketch with its textual description.





\paragraph{Data preparation}
We randomly select $10k$ photos from MS-COCO \cite{lin2014cocoCaption}, a standard benchmark dataset for scene understanding \cite{CLIP, deeplabv2, chen2021visualgpt}. Each photo is accompanied by image captions \cite{lin2014cocoCaption} and semantic segmentation \cite{caesar2018cocostuff}.
Our selected subset of photos includes $72$ \emph{``things"} instances (well-defined foreground objects) and $78$ \emph{``stuff"} instances (background instances with potentially no specific or distinctive spatial extent or shape: e.g., ``trees", ``fence"), according to the classification introduced in \cite{caesar2018cocostuff}.

\paragraph{Task}
We built a custom web application\footnote{We will release the code for the annotation tool and backend-server script upon acceptance.} to engage $100$ participants, each annotating a distinct subset of $100$ photos.
%
Our objective is to collect easy-to-recognize freehand scene sketches drawn from memory, alike single-object sketches collected previously \cite{tu-berlin, sketchy}.
To imitate real world scenario of sketching from memory, following the practice of single object dataset collection, we showed a reference scene photo to a subject for a limited duration of $60$ seconds.
To ensure recognizable, but not overly detailed drawings, we also imposed time constraints on the duration of the sketching. 
We determined the optimal time limits through a series of pilot studies with 10 participants, which showed that 3 minutes were sufficient for participants to comfortably sketch recognizable scene sketches.
%
% , then replaced it with the instructions: \emph{``Sketch the scene that you saw within $180$ seconds"}. 
% Users were able to start drawing by clicking \emph{the button to proceed}, which loads a blank canvas and a timer counting down from $180$. 
%
% We showed a reference scene photo to a subject for $60$ seconds, then replaced it with the instructions: \emph{``Sketch the scene that you saw within $180$ seconds"}. 
% Users were able to start drawing by clicking \emph{the button to proceed}, which loads a blank canvas and a timer counting down from $180$. 
Repeated sketching trials were allowed, with a subject making {$1.7$} trials on average. Each trial repeats the entire process of viewing and sketching from a blank canvas.
%
To reduce fatigue that can compromise data quality, we encourage participants to take frequent breaks and complete the task over multiple days. 
Hence, each participant spent $12-13$ hours to annotate $100$ photos over an average period of $2$ days.

Upon satisfaction with their sketch, we ask the same subject to describe their sketch in text, where instructions\footnote{We provide the detailed instructions in the Supplemental.} to write a sketch caption are similar to that of Lin \etal \cite{lin2014cocoCaption}. 
% We ask the same subject to write a sketch caption. This ensures consistency of salient information in the sketch and the corresponding caption, avoiding misinterpretation of abstract scene sketches.



Finally, to perform sketches quality check, we hired one dedicated person as a \emph{human judge} (1) with experience in data collection and (2) non-expert in sketching.
A human judge was tasked with the instruction: \emph{``flag scene sketches that are too difficult to understand or recognize"}. 
The \emph{flagged} photos were sent back to their assigned annotator. 
This process guarantees the resulting scene sketches are recognizable by a human, and hence in principle, should be understood by a machine.



\paragraph{Participants}
We recruited $100$ participants, non-experts in sketching, from the age group $22-44$, with the mean age of $27.03$, comprising $72$ males and $28$ females\footnote{See supplemental for details on how consent was obtained.}. 

\paragraph{Dataset composition}
Our dataset consists of $10,000$ (a) unique freehand scene sketches, (b) textual descriptions of the sketches (sketch captions), (c) reference photos from the MS-COCO \cite{lin2014cocoCaption} dataset.
Each photo in \cite{lin2014cocoCaption} contains 5 associated text descriptions (image captions) by different subjects \cite{lin2014cocoCaption}. \cref{fig:sample-data} provides some examples, while \cref{tab:datasets_comparison} provides comparison with previous dataset and statistics on distribution of object categories in our sketches. 
The supplemental provides additional sketch examples and detailed statistics on object categories.



==> eccv_copy/intro.tex <==
\begin{figure}[!h]
    \centering
    \includegraphics[width=\linewidth]{./images/dataset-comparison_v3.pdf}
    \caption{
	 Existing datasets of scene sketches \texttt{SketchyCOCO} \cite{gao2020sketchyCOCO} are obtained by synthetically combining sketches of individual objects. This can sometimes lead to non-representative sketches. Distinctively, our dataset of freehand scene sketches exhibits object and scene level abstraction. Moreover, the sketches in our dataset contain temporal strokes order information. We visualize the strokes order using the ``Parula" color scheme: strokes in ``blue" are drawn first, strokes in ``yellow" are drawn last. \cut{Choose more interesting sketches for our dataset, I think we can also show just two sketches from the previous datasets and 6 for our dataset. For SketchyCOCO and ours can we show sketches for the same images?}      
}
    \label{fig: dataset-comparison}
    \vspace{-0.6cm}
\end{figure}

\section{Introduction}
\label{sec:intro}

As research on sketching thrives \cite{ha2018quickdraw, sketchy, tu-berlin, bhunia2020pixelor}, the focus shifts from an analysis of  quick single-object sketches to an analysis of scene sketches \cite{sketchyscene, gao2020sketchyCOCO, liu2020scenesketcher}, and professional \cite{lift3d} or specialised \cite{garmentdesign_Wang_SA18} sketches.
%
In the age of data-driven computing, conducting research on sketching requires representative datasets.
% comprising of freehand sketches. 
For instance, the inception of object-level sketch datasets \cite{ha2018quickdraw, text-sketch, yu2016shoe, sketchy, tu-berlin, 2019opensketch} enabled and propelled research in diverse applications \cite{bhunia2020pixelor, sketchSelf, beziersketch}. Recently, increasingly more attempts are conducted towards not only collecting the data but also understanding how humans sketch \cite{2019opensketch, bhunia2020pixelor, whyLineDrawings, 2020:ABR, 2021Tracing}. We extend these efforts to scene sketches by introducing \newDataset, the first dataset of $10,000$ unique freehand scene sketches, drawn by $100$ non-expert participants. 
%
We envision this dataset to permit a multitude of novel tasks and to contribute to the fundamental understanding of visual abstraction and expressivity in scene sketching. With our work, we make the first stab in this direction: We study the role of freehand sketches in fine-grained image retrieval and sketch understanding on the example of sketch-captioning.


Thus far, research on scene sketches leveraged semi-synthetic \cite{gao2020sketchyCOCO, liu2020scenesketcher, sketchyscene} datasets that are obtained by combining together sketches and clip-arts of individual objects. 
Such datasets lack the holistic scene-level abstraction that characterises real scene sketches. 
Fig.~\ref{fig: dataset-comparison} shows a visual comparison between existing semi-synthetic \cite{gao2020sketchyCOCO,sketchyscene} scene sketch datasets and ours \newDataset. 
\new{It shows complex interactions between scene elements in our sketches and diversity of objects depictions. 
Moreover, our sketches contain more object categories than previous datasets: Our sketches contain 95 categories from the COCO-stuff \cite{caesar2018cocostuff}, while sketches in SketchyScene \cite{sketchyscene} and  SketchyCOCO \cite{gao2020sketchyCOCO} contain 45 and 17 object categories, respectively.} 

Our dataset collection setup is practical applications-driven, such as the retrieval of a video frame given a quick sketch from memory. Our objective is to collect easy to recognize quick freehand scene sketches from memory (similar to object sketches collected previously \cite{tu-berlin, sketchy}). 
To ensure recognisable but not too detailed sketches we impose a 3-minutes sketching time constraint, where the optimal time duration was determined through a series of pilot studies.  
A scene reference photo is shown to a subject for $60$ seconds before being asked to sketch from memory. We record time-space coordinates of each sketch stroke. 
As reference images, we select photos from the MS-COCO \cite{lin2014cocoCaption}, a benchmark dataset for scene understanding, that ensures diversity of scenes and is complemented with rich annotations in a form of semantic segmentation and image captions. 

Equipped with our \newDataset{} dataset, we for the first time study the problem of a fine-grained image retrieval from freehand scene sketches. 
First, we study how indicative is the performance observed through training and testing on semi-synthetic datasets \cite{sketchyscene, gao2020sketchyCOCO}, that are easier to collect, of the performance on freehand sketches from our dataset. 
Then, in our work we aim at understanding how scene-sketch-based retrieval compares to text-based retrieval, and what information sketch captures. To obtain a thorough understanding, we collect for each sketch its text description. The text description is done by the subject who created the sketch, eliminating the noise due to sketch interpretation. 
Such text description allows us to compare it with image text description from the MS-COCO \cite{lin2014cocoCaption} dataset, shedding light on the complementary nature of the two modalities.


Our dataset of freehand scene sketches enables analysis towards insights into how humans sketch scenes, not possible with earlier datasets \cite{gao2020sketchyCOCO}. We conduct such analysis in the context of the fine-grained retrieval. First, the diversity of user styles and large number of sketch instances for each of participants allows us to demonstrate the potential of personalization in sketch-related tasks. In particular, we adopt meta-learning \cite{maml, how-to-train-maml} to increase the accuracy of the retrieval for a particular subject given a few sketch examples, capturing abstraction specific to this subject.
Second, we continue the recent trend on understanding and leveraging strokes order \cite{2019opensketch, bhunia2020pixelor, lift3d, 2021Tracing} and observe the same trends of coarse-to-fine sketching in scene sketches. Notably, we study salience of early versus latter strokes for the retrieval task. Finally, we study the task of sketch-captioning contributing towards sketch understanding. 


Collecting human sketches is costly, and despite our dataset is relatively large-scale, it is hard to reach the scale of the existing datasets of photos \cite{witdataset, conceptual-captions, SBU-captions}. To tackle this known problem of sketch data, recent work \cite{sketchJigsaw, sketchSelf} to improve the performance of the encoder-decoder-based architectures on the downstream tasks proposed to pre-train the encoder relying on some auxiliary task. They showed that this strategy is beneficial over pre-training on photos. 
Last but not least, in our work we build on \cite{sketchSelf} and consider the auxiliary task of raster sketch to vector sketch generation. Since our sketches are more complex than those of single objects considered before, we propose a dedicated hierarchical RNN decoder. We demonstrate the efficiency of the pre-training strategy and our proposed hierarchical decoder on the fine-grained retrieval and sketch-captioning tasks.

In summary, our contributions are: (1) We propose the first dataset of freehand scene sketches and their captions; (2) We study for the first time fine-grained freehand-scene-sketch-based image retrieval (3) and the relations between sketches, images and their captions. 
(4) Contributing to sketch understanding, we study personalization with meta-learning, strokes salience and sketch-captioning tasks.
(5) Finally, to address the challenges of scaling sketch datasets and complexity of scene sketches, we introduce a novel hierarchical sketch decoder. We leverage this decoder at the pre-training stage for the fine-grained retrieval and sketch captioning tasks.

==> eccv_copy/related_work.tex <==
\begin{table*}[ht]
    \centering
    \caption{Comparison of scene sketch datasets: \texttt{SketchyScene} \cite{sketchyscene}, \texttt{SketchyCOCO} \cite{gao2020sketchyCOCO} and \newDataset. We use the semantic segmentation labels to compute the statistics on categories present in \cite{sketchyscene,gao2020sketchyCOCO}. 
    For our dataset, we look for the occurrence of one of COCO-Stuff \cite{caesar2018cocostuff} categories in sketch captions. Our dataset is well-balanced, 95 categories are uniformly distributed among sketches with the lowest standard deviation among the datasets.}
    \vspace{-0.25cm}
    \small{
\resizebox{\linewidth}{!}{%
\begin{tabular}{c|cc|r|c|c|c|r|rrrr|rrrr}
\hline\hline
\multirow{2}{*}{Dataset} & \multicolumn{2}{c|}{Abstraction} & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}$\#$ pho-\\ tos\end{tabular}}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Vector \\ Sketch\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Cap-\\ tions\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Free-\\ hand\end{tabular}} & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}$\#$cate-\\ gories\end{tabular}}} & \multicolumn{4}{c|}{$\#$ categories per sketch}                                                           & \multicolumn{4}{c}{$\#$ sketches per category}                                                              \\
                         & Object          & Scene          & \multicolumn{1}{c|}{}                                                                         &                                                                           &                                                                       &                                                                       & \multicolumn{1}{c|}{}                                                                            & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c|}{Std}  & \multicolumn{1}{c}{Min} & \multicolumn{1}{c|}{Max} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c|}{Std}     & \multicolumn{1}{c}{Min} & \multicolumn{1}{c}{Max} \\ \hline
\texttt{SketchyScene}    & \textcolor{PineGreen}{\cmark}         & \xmark         & 7,264                                                                                         & \xmark                                                                    & \xmark                                                                & \xmark                                                                & 45                                                                                               & 7.88                     & \multicolumn{1}{r|}{1.96} & 4                       & 20                       & 1087.02                  & \multicolumn{1}{r|}{1416.49} & 31                      & 5723                    \\
\texttt{SketchyCOCO}     & \xmark          & \textcolor{PineGreen}{\cmark}        & 14,081                                                                                        & \xmark                                                                    & \xmark                                                                & \xmark                                                                & 17                                                                                               & 3.33                     & \multicolumn{1}{r|}{0.9}  & 2                       & 7                        & 1932.41                  & \multicolumn{1}{r|}{3388.72} & 33                      & 9761                    \\
\textbf{FS-COCO (ours)}  & \textcolor{PineGreen}{\cmark}         & \textcolor{PineGreen}{\cmark}        & 10,000                                                                                        & \textcolor{PineGreen}{\cmark}                                                                   & \textcolor{PineGreen}{\cmark}                                                               & \textcolor{PineGreen}{\cmark}                                                               & 95                                                                                               & 1.37                     & \multicolumn{1}{r|}{0.57} & 1                       & 5                        & 89.72                    & \multicolumn{1}{r|}{159.9}   & 1                       & 853                     \\ \hline
\end{tabular}%
}
    }
    \label{tab:datasets_comparison}
     \vspace{-0.3cm}
\end{table*}


\section{Related Work}
\label{sec:related_work}

\paragraph{Single-Object Sketch Datasets}
Most freehand sketch datasets contain sketches of individual objects, annotated at the category level \cite{tu-berlin, ha2018quickdraw} or part level \cite{ge2021creative}, or have paired photos \cite{yu2016shoe, sketchy, text-sketch} or 3D shapes \cite{sketch_3Dshape_2021}. 
Category-level and part-level annotations enable tasks such as sketch recognition \cite{sketch-a-net, sketch-classification2014} and sketch generation \cite{ge2021creative, bhunia2020pixelor}. 
\emph{Paired} datasets allow to study practical tasks such as sketch-based image retrieval \cite{yu2016shoe} and sketch-based image generation \cite{sketchGan}.

However, collecting fine-grained paired datasets is time-consuming since one needs to ensure accurate, fine-grained matching while keeping the sketching task natural for the subjects \cite{reference-drawing}. Hence, such paired datasets typically contain a few thousand sketches per category, \eg, {QMUL-Chair-V2} \cite{yu2016shoe} consists of $1432$ sketch-photo pairs on a single `chair' category, {Sketchy} \cite{sketchy} has an average of $600$ sketches per category, albeit over $125$ categories.

In contrast, our dataset contains \emph{10,000 scene} sketches, each paired with a `reference' photo and text description. 
It contains scene sketches that are more challenging to collect and excels the existing fine-grained datasets of single-object sketches in the amount of paired instances.
%Apart from providing freehand scene sketches that are more challenging to collect, our proposed dataset has more instances of paired sketch-photo-text than existing object-sketch datasets with paired sketch-photo from a single category. 
It will foster research on scene-sketch-understanding, retrieval, and diverse generative tasks (\eg, sketch-based image generation).





\paragraph{Scene Sketch Datasets}
\new{A dataset of 8,694 freehand scene sketches was collected within the multi-model dataset \cite{ayatar2016crossmodal}. 
It contains sketches of 205 scenes, but the examples are not paired between modalities.}
While scene sketch datasets with pairing between modalities \cite{sketchyscene,gao2020sketchyCOCO} have recently started to appear, these are \emph{`semi-synthetic'}. 
%{SketchyScene} \cite{sketchyscene} introduced the first scene sketch dataset with $7,264$ sketch `templates' created by humans via \emph{drag-and-drop} of {clip-art like} object sketches. 
%{SketchyCOCO} \cite{gao2020sketchyCOCO} synthesized scene sketches by spatially arranging object sketches from {Sketchy} using semantic segmentation maps of photos in COCO Stuff \cite{caesar2018cocostuff}.
Thus, the {SketchyScene} \cite{sketchyscene} dataset contains $7,264$ sketch-image pairs. It is obtained by providing participants with a reference image and clip-art like object sketches to drag-and-drop for scene composition. The augmentation is performed by replacing object sketches with other sketch instances belonging to the same object category.
{SketchyCOCO} \cite{gao2020sketchyCOCO} was generated automatically relying on the segmentation maps of photos from COCO-Stuff \cite{caesar2018cocostuff}, and leveraging freehand sketches of single objects from \cite{sketchy,tu-berlin,ha2018quickdraw}.
Unlike existing semi-synthetic datasets, our dataset of freehand scene sketches captures abstraction on the intrinsic object level and holistic scene level (\cref{tab:datasets_comparison}). 
% Exceptionally, our data enables us to study the domain gap between previously introduced semi-synthetic sketches and freehand scene sketches.



\paragraph{Sketch Understanding}
The lack of freehand scene sketch datasets severely limits the proliferation of research on scene sketch understanding. 
Nevertheless, leveraging the semi-synthetic datasets previous work studied scene sketch semantic segmentation \cite{sketchyscene}, scene-level fine-grained sketch based image retrieval \cite{liu2020scenesketcher}, and image generation \cite{gao2020sketchyCOCO}.
%
Uniquely, our goal is to enable the analysis of \emph{freehand} scene sketches.
Following the footstep of understanding scenes in photos\cite{xu2015show,wang2017agcvae, mahajan2020lnfmm}, we study sketch captioning for the first time using the paired sketch-text instances available in our dataset.

%Nevertheless, leveraging the semi-synthetic dataset {SketchyScene} \cite{sketchyscene}, Zou \etal \cite{sketchyscene} performed scene sketch semantic segmentation using a customized DeepLab-V2 network \cite{deeplabv2}. 
%Later, Liu \etal \cite{liu2020scenesketcher} proposed a complex graph-based embedding method for scene-level fine-grained sketch based image retrieval using object-level annotations for sketches and photos in {SketchyCOCO} \cite{gao2020sketchyCOCO}. 
%In contrast to understanding semi-synthetic sketches \cite{sketchyscene, gao2020sketchyCOCO}, we enable the analysis of freehand scene sketches. In context of scene image understanding, image captioning \cite{xu2015show,wang2017agcvae, mahajan2020lnfmm} is widely recognized as the benchmark task. Following the footstep of understanding scenes in photos, we introduce sketch captioning for the first time using the paired sketch-text instances available in our dataset.

%
%\begin{figure*}[ht]
%    \centering
%    \includegraphics[width=\linewidth]{./images/sample-data.pdf}    
%    \vspace{-0.6cm}
%    \caption{Examples of our dataset of freehand scene sketches comprising fine-grained scene sketch, text, and photo paired information. Each sketch is available in a vector format with space-time information for each sketch point. A qualitative comparison of image- and sketch-captions: The overlapping words are marked in \textcolor{blue}{Blue}, the words present only in image-captions are marked in \textcolor{caption-red}{Red}, while the words present only in sketch-captions are marked in \textcolor{deepGreen}{Green}.
%    }
%    \label{fig:sample-data}
%    \vspace{-0.4cm}
%\end{figure*}





==> intro.tex <==
\section{Introduction}
\label{sec:intro}
\begin{figure}[!h]
    \centering
    \includegraphics[width=\linewidth]{./images/dataset-comparison_v5.pdf}
    % \vspace{-0.6cm}
    \caption{
% 	 Existing datasets of scene sketches \texttt{SketchyScene} \cite{sketchyscene} and \texttt{SketchyCOCO} \cite{gao2020sketchyCOCO} are obtained by combining together clip-arts and sketches of individual objects, respectively. 
	 Comparison of our sketches to the scene sketches from \texttt{SketchyCOCO}, the latter are obtained by combining together sketches of individual objects.
	 Our freehand scene sketches contain abstraction at the object and scene level and better capture the content of reference scenes.
	 This figure demonstrates a large domain gap between freehand scene sketches and available scene sketches, motivating the need for new datasets.
	 Our sketches contain stroke temporal order information, which we visualize using the ``Parula" color scheme: strokes in {\color{blue}``blue"} are drawn first, strokes in {\color{yellow}``yellow"} are drawn last.
}
    \label{fig:dataset-comparison}
    \vspace{-0.6cm}
\end{figure}



As research on sketching thrives \cite{ha2018quickdraw, sketchy, tu-berlin, bhunia2020pixelor}, the focus shifts from an analysis of  quick single-object sketches \cite{bhunia2022subset, bhunia2022diy, Sketch3T, bhunia2022adaptive} to an analysis of scene sketches \cite{sketchyscene, gao2020sketchyCOCO, liu2020scenesketcher, pinaki2022PartialSBIR}, and professional \cite{lift3d} or specialised \cite{garmentdesign_Wang_SA18} sketches.
%
In the age of data-driven computing, conducting research on sketching requires representative datasets.
% comprising of freehand sketches. 
For instance, the inception of object-level sketch datasets \cite{ha2018quickdraw, text-sketch, yu2016shoe, sketchy, tu-berlin, 2019opensketch} enabled and propelled research in diverse applications \cite{bhunia2020pixelor, sketchSelf, beziersketch}. Recently, increasingly more attempts are conducted towards not only collecting the data but also understanding how humans sketch \cite{2019opensketch, bhunia2020pixelor, whyLineDrawings, 2020:ABR, 2021Tracing}. 
We extend these efforts to scene sketches by introducing \newDataset{} (Freehand Sketches of Common
Objects in COntext), the first dataset of $10,000$ unique freehand scene sketches, drawn by $100$ non-expert participants. 
%
We envision this dataset to permit a multitude of novel tasks and to contribute to the fundamental understanding of visual abstraction and expressivity in scene sketching. With our work, we make the first stab in this direction: 
We study fine-grained image retrieval from freehand scene sketches and the task of scene sketch captioning.


Thus far, research on scene sketches leveraged semi-synthetic \cite{gao2020sketchyCOCO, liu2020scenesketcher, sketchyscene} datasets that are obtained by combining together sketches and clip-arts of individual objects. 
Such datasets lack the holistic scene-level abstraction that characterises real scene sketches. 
Fig.~\ref{fig:dataset-comparison} shows a visual comparison between the existing semi-synthetic \cite{gao2020sketchyCOCO} scene sketch dataset and ours \newDataset. 
It shows interactions between scene elements in our sketches and diversity of objects depictions. 
Moreover, our sketches contain more object categories than previous datasets: Our sketches contain more than 92 categories from the COCO-stuff \cite{caesar2018cocostuff}, while sketches in SketchyScene \cite{sketchyscene} and  SketchyCOCO \cite{gao2020sketchyCOCO} contain 45 and 17 object categories, respectively.

Our dataset collection setup is practical applications-driven, such as the retrieval of a video frame given a quick sketch from memory. 
\new{This is an important task because, while the text-based retrieval achieved impressive results in recent years, it might be easier to communicate via sketching fine-grained details.
However, this will only be practical if users can provide a quick sketch and are not expected to be good sketchers.}
Therefore, we collect \emph{easy to recognize but quick to create} freehand scene sketches from recollection (similar to object sketches collected previously \cite{tu-berlin, sketchy}). 
As reference images, we select photos from the MS-COCO \cite{lin2014cocoCaption}, a benchmark dataset for scene understanding, that ensures diversity of scenes and is complemented with rich annotations in a form of semantic segmentation and image captions. 

Equipped with our \newDataset{} dataset, we for the first time study the problem of a fine-grained image retrieval from freehand scene sketches. 
First, we study how indicative is the performance observed through training and testing on semi-synthetic datasets \cite{sketchyscene, gao2020sketchyCOCO}, that are easier to collect, of the performance on freehand sketches.
Then, in our work we aim at understanding how scene-sketch-based retrieval compares to text-based retrieval, and what information sketch captures. To obtain a thorough understanding, we collect for each sketch its text description. 
The text description makes the subject who created the sketch, eliminating the noise due to sketch interpretation. 
By comparing sketch text descriptions with image text descriptions from the MS-COCO \cite{lin2014cocoCaption} dataset, we draw conclusions on the complementary nature of the two modalities: sketches and image text descriptions.


Our dataset of freehand scene sketches enables analysis towards insights into how humans sketch scenes, not possible with earlier datasets \cite{gao2020sketchyCOCO}. 
We continue the recent trend on understanding and leveraging strokes order \cite{2019opensketch, bhunia2020pixelor, lift3d, 2021Tracing} and observe the same trends of coarse-to-fine sketching in scene sketches: We study stroke order as a factor of its salience for retrieval. 
Finally, we study sketch-captioning as an example of a sketch understanding task. 


Collecting human sketches is costly, and despite our dataset being relatively large-scale, it is hard to reach the scale of the existing datasets of photos \cite{witdataset, conceptual-captions, SBU-captions}. To tackle this known problem of sketch data, recent work \cite{sketchJigsaw, sketchSelf} to improve the performance of the encoder-decoder-based architectures on the downstream tasks proposed to pre-train the encoder relying on some auxiliary task. They showed that this strategy is beneficial over pre-training on photos. 
Last but not least, in our work we build on \cite{sketchSelf} and consider the auxiliary task of raster sketch to vector sketch generation. Since our sketches are more complex than those of single objects considered before, we propose a dedicated hierarchical RNN decoder. We demonstrate the efficiency of the pre-training strategy and our proposed hierarchical decoder on fine-grained retrieval and sketch-captioning.

In summary, our contributions are: (1) We propose the first dataset of freehand scene sketches and their captions; (2) We study for the first time fine-grained freehand-scene-sketch-based image retrieval (3) and the relations between sketches, images and their captions. 
% (4) Contributing to sketch understanding, we study personalization with meta-learning, strokes salience and sketch-captioning tasks.
(4) Finally, to address the challenges of scaling sketch datasets and complexity of scene sketches, we introduce a novel hierarchical sketch decoder that exploit temporal stroke order available for our sketches. 
We leverage this decoder at the pre-training stage for fine-grained retrieval and sketch captioning.
 
 

%brings additional annotation such semantic segmentation and image captions (textual description of photo).
% Sketches are distinct from photos that are created by humans through an iterative process and reflect one's sketching skills, taste, perception, and creativity. Pertinent research in child psychology, cross-cultural psychology, and animal psychology have acknowledged the universality of this form of expression without the need of having prior knowledge \cite{picture-perception}. This motivated sketches as an attractive interface for human computer interaction \cite{cassie} thereby opening computing technology to a significantly larger user base than text input alone. With inception of object-level sketch datasets \cite{ha2018quickdraw, text-sketch, yu2016shoe, sketchy, tu-berlin}, research into human drawn objects have shown a tremendous growth \cite{bhunia2020pixelor, sketchSelf, beziersketch}. However, in the age of data-driven computing the lack of readily available human drawn scene sketch dataset has created a barrier to applications using sketched scenes and our fundamental understanding of visual abstraction and expressivity.


%A naive solution to this barrier of sketching for downstream applications \cite{garmentdesign_Wang_SA18} is employing non-photorealistic rendering \cite{suggestiveContours} or line drawings \cite{photosketching}. 
%%However, its lack of realism \cite{whyLineDrawings} has motivated works targeting real world sketches \cite{lift3d}.
%\refactor{The overwhelming need for real world sketches motivated works such as \texttt{SketchyScene} \cite{sketchyscene} and \texttt{SketchyCOCO} \cite{gao2020sketchyCOCO} to propose ``scene" sketches but such sketches do not fall into our definition of what constitutes scene-sketches -- they are more ``image-like", and synthetically generated by randomly placing \emph{object sketches} of different styles and abstraction level onto existing \emph{image scene-templates}.} 
%Thus they do not form a good basis for our general mission on human scene understanding. 
%%A visual comparison of such ``template" scene sketches vs. our free-hand scene sketches can be found in Fig. \ref{fig:dataset-comparison}.


% Zou \etal \cite{sketchyscene} that proposed a dataset which \emph{drag-and-drops} ``clip-art" like objects sketches to capture abstraction only in scene-level. Gao \etal \cite{gao2020sketchyCOCO} synthesised a dataset using free-hand object sketches arranged in a scene following the semantic segmentation mask of a photo. However, none of these existing artificial datasets represent the iterative sketching process by an amature that leads to a holistic free-hand scene sketch (see Fig. \ref{fig:dataset-comparison}) showing abstraction on both object- and scene-level.

% Introduce our dataset in brief and salient points. How ours capture both object- and scene-level abstraction. In addition to support numerous application we capture paired text caption. We purposefully choose our images from MS-COCO dataset which provides makes a wide range of annotations available to the community with semantic segmentation, instance segmentation, image-captions among others.

%We introduce the first free-hand scene sketch dataset, \texttt{HumanSketch} comprising of $10,000$ human drawn scene sketches. For this, we recruited $100$ self-reported non-expert participants. 
%Our objective is to collect \refactor{easy to recognize hand drawn scene sketches from memory (akin to object sketches \cite{tu-berlin, sketchy}) that supports important downstream applications such as free-hand scene fine-grained sketch-based image retrieval (FG-SBIR) among others}. 
%
%Based on a pilot study, our servers time-bound the drawing process to prevent annotators from rushing or over-exaggerations. Our servers additionally recorded vectored coordinate information and textual description of scene sketches (sketch captions) to maximise possible downstream applications. We select our photos from the benchmark scene understanding dataset MS-COCO \cite{lin2014cocoCaption} which apart from ensuring scene diversity brings additional annotation such semantic segmentation and image captions (textual description of photo).

% Talk about applications: fine-grianed free-hand scene sketch-based image retrieval and why it was not done before. Talk about sketch captioning and in spite of being mentioned before as a wishful research direction, there was no dataset or annotations to support such research. What can scene sketch say that images can't? We .....

%Our novel dataset provides fine-grained information in sketch, text, and photo modalities. We for the first time study the problem of free-hand scene FG-SBIR. Comparing our \texttt{HumanSketch} with ``image-like" scene sketch datasets \cite{sketchyscene, gao2020sketchyCOCO} reveal whether a higher performance on synthetic sketches generalise to the practical scenario with human drawn sketches as input. Motivated by paired textual description of scene sketches we introduce sketch captioning. While prior research \cite{sketchyscene} had quoted it as part of interesting future research, there exists no practical manifestation due to lack of an appropriate dataset. A hierarchical decoder is proposed to enable sketch-specific pre-training strategy that alleviates the added complexity posed by scene sketches with object- and scene-level abstraction. As byproduct of our novel sketch decoder, we show some preliminary qualitative results on photo-to-sketch synthesis. Our user-level annotation permits personalised AI via meta-adaptation to user-specific sketches. Apart from practical applications, our novel dataset also serves as a key enabler in the fundamental understanding of visual abstraction and expressivity. We provide a quantitative measure of \emph{how much salient are initial human drawn strokes} by measuring FG-SBIR performance of SOTA \cite{yu2016shoe} models by masking strokes near beginning or end in the iterative human sketching process. While sketches have been recognised as a superior query modality than text for fine-grained image retrieval \cite{text-sketch}, comparing image-captions, free-hand scene sketches, and sketch-captions together provides insights to what makes sketches superior to text for retrieval. Our multi-modal dataset also enables studying the complimentary nature of sketches and text via sketch+text combined fine-grained image retrieval.

%In summary, our contributions are: (a) we propose a novel free-hand scene sketches and their captions to facilitate the study on fine-grained cross-modal scene understanding. (b) Using this dataset we study for the first time free-hand scene fine-grained sketch-based image retrieval (c) and introduce sketch captioning. (d) To address the added complexity of scene sketches we introduce a novel hierarchical sketch decoder that supports a sketch-specific pre-training strategy  (e) our novel dataset reveals several interesting insights to inform future research.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> related_work.tex <==



\section{Related Work}
\label{sec:related_work}

\paragraph{Single-Object Sketch Datasets}
Most freehand sketch datasets contain sketches of individual objects, annotated at the category level \cite{tu-berlin, ha2018quickdraw} or part level \cite{ge2021creative}, paired to photos \cite{yu2016shoe, sketchy, text-sketch} or 3D shapes \cite{sketch_3Dshape_2021}. 
Category-level and part-level annotations enable tasks such as sketch recognition \cite{sketch-a-net, sketch-classification2014} and sketch generation \cite{ge2021creative, bhunia2020pixelor}. 
\emph{Paired} datasets allow to study practical tasks such as sketch-based image retrieval \cite{yu2016shoe} and sketch-based image generation \cite{sketchGan}.

However, collecting fine-grained paired datasets is time-consuming since one needs to ensure accurate, fine-grained matching while keeping the sketching task natural for the subjects \cite{reference-drawing}. Hence, such paired datasets typically contain a few thousand sketches per category, \eg, {QMUL-Chair-V2} \cite{yu2016shoe} consists of $1432$ sketch-photo pairs on a single `chair' category, {Sketchy} \cite{sketchy} has an average of $600$ sketches per category, albeit over $125$ categories.

Our dataset contains \emph{10,000 scene sketches}, each paired with a `reference' photo and text description. 
It contains scene sketches rather than sketches of individual objects and excels the existing fine-grained datasets of single-object sketches in the amount of paired instances.
%Apart from providing freehand scene sketches that are more challenging to collect, our proposed dataset has more instances of paired sketch-photo-text than existing object-sketch datasets with paired sketch-photo from a single category. 
% 





\paragraph{Scene Sketch Datasets}
Probably the first dataset of 8,694 freehand scene sketches was collected within the multi-model dataset \cite{ayatar2016crossmodal}. 
It contains sketches of 205 scenes, but the examples are not paired between modalities.
Scene sketch datasets with the pairing between modalities \cite{sketchyscene,gao2020sketchyCOCO} have started to appear, however they are \emph{`semi-synthetic'}. 
%{SketchyScene} \cite{sketchyscene} introduced the first scene sketch dataset with $7,264$ sketch `templates' created by humans via \emph{drag-and-drop} of {clip-art like} object sketches. 
%{SketchyCOCO} \cite{gao2020sketchyCOCO} synthesized scene sketches by spatially arranging object sketches from {Sketchy} using semantic segmentation maps of photos in COCO Stuff \cite{caesar2018cocostuff}.
Thus, the {SketchyScene} \cite{sketchyscene} dataset contains $7,264$ sketch-image pairs. 
It is obtained by providing participants with a reference image and clip-art like object sketches to drag-and-drop for scene composition. The augmentation is performed by replacing object sketches with other sketch instances belonging to the same object category.
{SketchyCOCO} \cite{gao2020sketchyCOCO} was generated automatically relying on the segmentation maps of photos from COCO-Stuff \cite{caesar2018cocostuff} and leveraging freehand sketches of single objects from \cite{sketchy,tu-berlin,ha2018quickdraw}.

Leveraging the semi-synthetic datasets, previous work studied scene sketch semantic segmentation \cite{sketchyscene}, scene-level fine-grained sketch based image retrieval \cite{liu2020scenesketcher}, and image generation \cite{gao2020sketchyCOCO}.
Nevertheless, sketches in the existing datasets are not representative of freehand human sketches as shown in \cref{fig:dataset-comparison}, and therefore the existing results can be only considered preliminary.
%
Unlike existing semi-synthetic datasets, our dataset of freehand scene sketches captures abstraction at the object level and holistic scene level, and contains stroke temporal information.  
We provide a comparative statistics with previous datasets in \cref{tab:datasets_properties}, discussed in \cref{sec:compare}. 

\begin{table*}[t]
    \centering
    \caption{Properties of scene sketch datasets.}
%    \vspace{-0.25cm}
\scriptsize{
% \resizebox{\linewidth}{!}{%
\begin{tabular}{c|cc|r|c|c|c}
\multirow{2}{*}{Dataset} & \multicolumn{2}{c|}{Abstraction} & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}$\#$ pho-\\ tos\end{tabular}}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Vector \\ Sketch\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Cap-\\ tions\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Free-\\ hand\end{tabular}} \\
                         & Object          & Scene          & \multicolumn{1}{c|}{} & & & \\ \hline
\texttt{SketchyScene  \cite{sketchyscene}}    & \textcolor{PineGreen}{\cmark}         & \xmark         & 7,264                                                                                         & \xmark                                                                    & \xmark                                                                & \xmark                                                                 \\
\texttt{SketchyCOCO} \cite{gao2020sketchyCOCO}    & \xmark          & \textcolor{PineGreen}{\cmark}        & 14,081                                                                                        & \xmark                                                                    & \xmark                                                                & \xmark                                                                \\
\textbf{FS-COCO}  & \textcolor{PineGreen}{\cmark}         & \textcolor{PineGreen}{\cmark}        & 10,000                                                                                        & \textcolor{PineGreen}{\cmark}                                                                   & \textcolor{PineGreen}{\cmark}                                                               & \textcolor{PineGreen}{\cmark}                                                               \\ \hline
\end{tabular}%
% }
 }
    \label{tab:datasets_properties}
     \vspace{-0.3cm}
\end{table*}


The primary goal of our work is to provide a dataset of diverse freehand scene sketches to support the research on scene sketch understanding, retrieval, and diverse generative tasks (\eg, sketch-based image generation).
We demonstrate the benefit and importance of the newly proposed data on two problems: image retrieval and sketch captioning.
% The lack of freehand scene sketch datasets severely limits the proliferation of research on scene sketch understanding. 
% Uniquely, our goal is to enable the analysis of \emph{freehand} scene sketches.
% Following the footstep of understanding scenes in photos\cite{xu2015show,wang2017agcvae, mahajan2020lnfmm}, we study sketch captioning for the first time using the paired sketch-text instances available in our dataset.




% Exceptionally, our data enables us to study the domain gap between previously introduced semi-synthetic sketches and freehand scene sketches.




% \paragraph{Sketch Understanding}
% The lack of freehand scene sketch datasets severely limits the proliferation of research on scene sketch understanding. 
% Nevertheless, leveraging the semi-synthetic datasets previous work studied scene sketch semantic segmentation \cite{sketchyscene}, scene-level fine-grained sketch based image retrieval \cite{liu2020scenesketcher}, and image generation \cite{gao2020sketchyCOCO}.
% %
% Uniquely, our goal is to enable the analysis of \emph{freehand} scene sketches.
% Following the footstep of understanding scenes in photos\cite{xu2015show,wang2017agcvae, mahajan2020lnfmm}, we study sketch captioning for the first time using the paired sketch-text instances available in our dataset.

%Nevertheless, leveraging the semi-synthetic dataset {SketchyScene} \cite{sketchyscene}, Zou \etal \cite{sketchyscene} performed scene sketch semantic segmentation using a customized DeepLab-V2 network \cite{deeplabv2}. 
%Later, Liu \etal \cite{liu2020scenesketcher} proposed a complex graph-based embedding method for scene-level fine-grained sketch based image retrieval using object-level annotations for sketches and photos in {SketchyCOCO} \cite{gao2020sketchyCOCO}. 
%In contrast to understanding semi-synthetic sketches \cite{sketchyscene, gao2020sketchyCOCO}, we enable the analysis of freehand scene sketches. In context of scene image understanding, image captioning \cite{xu2015show,wang2017agcvae, mahajan2020lnfmm} is widely recognized as the benchmark task. Following the footstep of understanding scenes in photos, we introduce sketch captioning for the first time using the paired sketch-text instances available in our dataset.

%
%\begin{figure*}[ht]
%    \centering
%    \includegraphics[width=\linewidth]{./images/sample-data.pdf}    
%    \vspace{-0.6cm}
%    \caption{Examples of our dataset of freehand scene sketches comprising fine-grained scene sketch, text, and photo paired information. Each sketch is available in a vector format with space-time information for each sketch point. A qualitative comparison of image- and sketch-captions: The overlapping words are marked in \textcolor{blue}{Blue}, the words present only in image-captions are marked in \textcolor{caption-red}{Red}, while the words present only in sketch-captions are marked in \textcolor{deepGreen}{Green}.
%    }
%    \label{fig:sample-data}
%    \vspace{-0.4cm}
%\end{figure*}




